Towards Inter-character Relationship-driven Story Generation

In this paper, we introduce the task of modeling interpersonal relationships for story generation. For addressing this task, we propose Relationships as Latent Variables for Story Generation, (ReLiSt). ReLiSt generates stories sentence by sentence and has two major components - a relationship selector and a story continuer. The relationship selector specifies a latent variable to pick the relationship to exhibit in the next sentence and the story continuer generates the next sentence while expressing the selected relationship in a coherent way. Our automatic and human evaluations demonstrate that ReLiSt is able to generate stories with relationships that are more faithful to desired relationships while maintaining the content quality. The relationship assignments to sentences during inference bring interpretability to ReLiSt.

==> old_intro.tex <==
Story generation is enriched via emotional relationships\fb{why emotional? inter-character}. They are integral to an engaging story. Importance of relationships to stories is well established \cite{bochner1997relationships}. However few study story generation from the perspective of character relationships. Most story generation works typically involve a plan detailing major events of the story \cite{rashkin-etal-2020-plotmachines,yao2019plan,goldfarb-tarrant-etal-2020-content} and can use linguistic instructions to condition the story on\cite{fan-etal-2018-hierarchical}. While these methods can generate stories based on diverse information, they are not trained to encode character relations directly. Hence, they provide weaker control over generation conditioned on relationships. In this paper We study relationship driven story generation. In this problem given a set of relationships, we aim to generate a story from which the input relationships can be inferred.

\sout{Why is this an important problem?
}Apart from importance of relationships, importance of an emotional story is also well recognized. Cognitive science studies \cite{parkinson1993making}, early rule based story generation \cite{y2007employing} and modern models \cite{brahman-chaturvedi-2020-modeling} all recognize the role of emotions at generating exciting stories.  

While relationships could be described in many ways, one of popular techniques to model the emotion of relationships is ``relationship polarity'' (RP). These works \cite{chaturvedi2016modeling,si-etal-2021-telling} consider relationships described as \textit{positive, negative or neutral}. The idea is that any or overall interaction between characters could be mapped to one of these three labels. The advantages relationship provides is that - 1. High frequency and universality of these terms implies that any sentence with the character mentions can be mapped to polarity. 2. Easier extraction as opposed to more fine grained relationships due to RP's similarity to sentiment labels under certain conditions. We exploit this connection between relationships and sentiment to create our dataset.

\sout{What has prior work done to solve this problem?}
While we are first to formulate and address this problem statement, story generation models are certainly capable of generating multi-character and multi-relation stories.
Charchter-centric story generation \cite{ammanabrolu2021automated,liu2020character,chandu-etal-2019-way} might generate salient relationships due to encoding character level information or persona. However, if relationships are not a part of this persona the model is left to guess them based on other information among the characters leading to a lack of control over the relationships. Furthermore, these models often recite a story biased towards a character's perspective. Proposed approach encodes relationships while maintaining 3rd person perspective.

\sout{Why is it challenging?
}
The reason this is a challenging task is because of the many ways relationships are exhibited in story sentences. Not all sentences will contribute to the relationships, arguably, most of the sentences continue and setup the events of the story. Apart from the challenges of story generation in general, these are the challenges of the problem statement exclusively. The model has to recognize and remember long range dependencies and decide \textbf{when} to exhibit a relationship and \textbf{which} relationship.  Furthermore, apart from when, the model has to simultaneously \textbf{exhibit the said relationship polarity correctly}. This is a hard problem by itself, akin to generating sentences with input sentiment \cite{wang2018sentigan} or argument generation based on stance \cite{schiller-etal-2021-aspect}. Both of these tasks might have to be done at any point far from the input relationships and multiple times if multiple relations. While modern language models are good at long range dependencies, they might suffer if the tasks are difficult. Finally, the task is also challenging because of lack of relationship annotated dataset and automatic evaluation metrics for relationship faithfulness.


\sout{How am I addressing those challenges?
} Proposed approach (\model) for relationship based story generation breaks down the aforementioned challenges with two major components. Firstly, we tackle long range dependency issues via controlling our sentence generation one sentence at a time. Secondly, we have a relation selector component to explicitly handle the \textbf{when} and \textbf{which} questions. This model will decide at each sentence if and which relationship should be used for conditioning sentence generation. Thirdly, we have a story continuer component to generate a sentence with relationship rich information conditioned on a specific relationship. Hence, exhibiting relationship correctly. Finally, we wrap both the components in a probabilistic framework where relationships are latent variables enabling us to train both the components with Expectation Maximization (EM). We create our own annotated dataset for training models for this task drawing parallels with sentiment analysis. For a better convergence of EM we initialize the components using sentence level annotation. \AR{skip this sentence?} This is important since EM is sensitive to initialization \cite{hu2015initializing}. For automatic evaluation of this task, we propose two metrics that give higher scores to the model which generates stories more faithful to input relationships. Furthermore, both the proposed metrics do not need any human written stories let alone annotated relationships.

% should I mention silver labelled data ?
% BAD INTRO , GIVING PRIORITY TO DATASET AND LMs OVER YOUR MODEL%%%%%%%%%%%%%%%%%%%%%%%%
%Story Generation has come a long way in NLP. Earlier models looked for improving fluency and grammatical correctness\SC{citation needed}. However with advent of language modeling, we can achieve higher level goals in Story Generation such as emotional arcs \cite{brahman-chaturvedi-2020-modeling}, or stories from generic prompts\cite{fan-etal-2018-hierarchical}. Many datasets, but control over relationships not guarantted by just presence. 
\SC{(removed) There are many story generation datasets and not all of them suffer from this problem. So this is a weak argument.}

%Example: Jennifer has a big exam tomorrow. She got so stressed, she pulled an all-nighter. She went into class the next day, weary as can be. Her teacher stated that the test is postponed for next week. Jennifer felt bittersweet about it.
%Such datasets have too less information if any, to model relationship, where information is both the narrative content and number of characters.
%By presenting the problem as a story generation from given set of character relationships, we can generate engaging stories with multiple characters with differing relations between them.% citations showing multiple relationships or multiple characters makes story interesting
%While character-centric story generation is popular\cite{}, Very few works have addressed this problem statement. As a result there are hardly few datasets with annotated relationship labels and corresponding stories to reflect them. We create our own annotation using sentiment analysis and named entity recognition to get silver labels
\SC{(removed) all of this is low level details. You probably won't talk about it in the intro, at least not this early.}% for the problem. We then present a probabilistic generative model to train our architecture where each sentence is ``generated'' by a latent relationship. 


==> old_related_worl.tex <==
\section{Related Work}
\SC{This section needs to be more smooth}
\FB{I haven't read this.}
% generic story generation
Early works on automatic story generation used symbolic planning \cite{perez2001mexica,porteous2009controlling,riedl2010narrative}\FB{I think this sentence is becoming very repetitive in papers.}. The idea of a plan of events for a story became a central idea for story generation as recent seq2seq storytelling models also employ it \cite{martin2018event,yao2019plan,fan-etal-2018-hierarchical,xu-etal-2018-skeleton,rashkin-etal-2020-plotmachines,goldfarb-tarrant-etal-2020-content}. Advent of large language models such as GPT-2 \cite{radford2019language} gave rise to text generators which could generate fluent stories \cite{qin-etal-2019-counterfactual,guan-etal-2020-knowledge}.

%with long range dependencies\SC{Are you sure you can claim "long range dependencies"?}.%\sout{Along with story generation datasets which have multi-character and multi-relationships, LMs should be able to generate relationship rich stories. However, a strong control over relationships is not guaranteed by just presence of relationships in training data. Models have to be designed specifically for the task of relationship driven story generation.} elesewhere % aristotle and plot machines once results are ready rashkin-etal-2020-plotmachines %\SC{throughout this paper I see a focus on "lack of data". It would be fine if this were a dataset paper. But this paper is not about solving the problem of "the lack of data". In fact, your silver data is clearly not a solution to this problem as shown by your own experiments. So why bring this up repeatedly?}  

\FB{How about using this outline: talking about the importance of relationship and characters level information in stories and conversations (here you can cite some of the inter-character rel works by snighda and others). The say that despite its importance only few works explored modeling them for story generation and conversation systems. (then bring those works here. You already have them in the second para). The somehow connect with generating text with specific emotions/sentiments for character (cite mine and the Weber et al. and any other).  }

%works which address charcter centric, persona based, personality based
\FB{this is not a correct use of "Despite". Despite doesn't come with "Also".} While story generation has focused strongly on a story line of events, character-centric generation is also gaining popularity. These works condition story generation with some character-level information \cite{liu2020character,chandu-etal-2019-way}.% A Character-Centric Neural Model for Automated Story Generation
In conversation systems and dialogue generation, character perspective is highly valued \cite{majumder-etal-2020-like,majumder-etal-2021-unsupervised,li-etal-2016-persona,oraby-etal-2018-controlling}. \newcite{brahman-chaturvedi-2020-modeling} propose a solution to generate stories conditioned on the protagonist's emotional arc. \newcite{si-etal-2021-telling} solve a story completion task conditioned on previous dialogue, a summary and character relationships. However, the idea there was that imbuing the model with relationship information improves the task of choosing better sentence completion candidates hence significantly different.
\begin{comment}
citet{liu2020character} propose story generation with ..% A Character-Centric Neural Model for Automated Story Generation
\cite{majumder-etal-2020-like} %Like hiking? you probably enjoy nature: Persona-grounded dialog with commonsense expansions.
\cite{majumder-etal-2021-unsupervised} %Unsupervised Enrichment of Persona-grounded Dialog with Background Stories.
Dialog system studies which learn character embeddings from corpus \cite{li-etal-2016-persona,oraby-etal-2018-controlling}
%relationship
\cite{kim-klinger-2019-frowning} %https://aclanthology.org/N19-1067.pdf Klinger paper
\cite{chaturvedi2017unsupervised}%Unsupervised learning of evolving relationships between literary characters
\cite{iyyer-etal-2016-feuding}%Feuding Families and Former Friends: Unsupervised Learning for Dynamic Fictional Relationships
\cite{srivastava2016inferring} %Inferring interpersonal relations in narrative summaries
\cite{chaturvedi2016modeling},%Modeling evolving relationships between characters in literary novels
Social networks \cite{labatut2019extraction}%Extraction and Analysis of Fictional Character Networks: A Survey
\end{comment}

% works which address relationships 
Inter-character relationship extraction has also gained popularity in narrative studies \cite{kim-klinger-2019-frowning,iyyer-etal-2016-feuding,srivastava2016inferring}. \citet{chaturvedi2017unsupervised,chaturvedi2016modeling} extract relationships between characters in novels. Extracted relationships could also be described as a social network of characters \cite{labatut2019extraction}.


% generation conditioned on sentiment
Outside narrative studies, our work is similar to problem statements which involve text generation conditioned on sentiment or emotion. Such as generating sentences from sentiment label \cite{wang2018sentigan}, generating arguments from stance \cite{schiller-etal-2021-aspect} and generating dialogues based on emotion \cite{zhou2018emotional,huang-etal-2018-automatic,zhou-wang-2018-mojitalk}.

%works using Expecation Maximation and latent variables
\FB{This para is focusing too much on EM. Instead you can say things like: "X propose a framework to learn latent Y for the task of Z." and avoid saying what happens in E and M steps.}
Using expectation-maximization for maximizing task objective a task is well established idea  \cite{dempster1977maximum}. \citet{chaturvedi-etal-2017-story} treat importance of aspects that influence choosing better story ending as latent variables. %Story Comprehension for Predicting What Happens Next 
\citet{zhou2020towards} treat explanations as latent variables to jointly train classification and explanation generation tasks. %E-step generates explanations and M-step uses the explanations to train the classifier.% Towards Interpretable Natural Language
%Understanding with Explanations as Latent Variable

\SC{There is a AAAI paper on character-centric story generation that needs to be cited. Ask Faeze. Also, there a  paper that was contemporary to Faeze's EMNLP paper on the same topic. Cite that also }
